signSGD: Compressed Optimisation for Non-Convex Problems

Training large neural networks requires distributing learning across multiple workers, where the cost of communicating gradients can be a significant bottleneck. signSGD alleviates this problem by transmitting just the sign of each minibatch stochastic gradient. We prove that it can get the best of both worlds: compressed gradients and SGD-level convergence rate. The relative $\ell_1/\ell_2$ geometry of gradients, noise and curvature informs whether signSGD or SGD is theoretically better suited to a particular problem. On the practical side we find that the momentum counterpart of signSGD is able to match the accuracy and convergence speed of Adam on deep Imagenet models. We extend our theory to the distributed setting, where the parameter server uses majority vote to aggregate gradient signs from each worker enabling 1-bit compression of worker-server communication in both directions. Using a theorem by Gauss we prove that majority vote can achieve the same reduction in variance as full precision distributed SGD. Thus, there is great promise for sign-based optimisation schemes to achieve fast communication and fast convergence. Code to reproduce experiments is to be found at https://github.com/jxbz/signSGD .

==> theorem/signSGDsmall.tex <==
  \begin{tcolorbox}[boxsep=0pt, arc=0pt,
    boxrule=0.5pt,
 colback=white]
\begin{restatable}[Non-convex convergence rate of small-batch 
\signSGD{}]{theorem}{signSGDsmalltheorem}\label{thm:signSGDsmall}
Run algorithm \ref{alg:signSGD} for $K$ iterations under Assumptions 1 to 3. Further, assume that the stochastic gradient noise distribution is unimodal and symmetric (e.g. Gaussian). Set the learning rate and mini-batch size (independently of step $k$) as
  \begin{equation*}
  \delta_k = \frac{1}{\sqrt{\norm{\vec L}_1K}} \qquad \qquad n_k = 1
  \end{equation*}
  Let $N$ be the cumulative number of stochastic gradient calls up to step $K$, i.e.\  $N = \text{O}(K)$. Let $B_k$ be the set of gradient components at step $k$ with large signal-to-noise ratio $S_i := \frac{|g_{k,i}|}{\sigma_i}$, i.e. $B_k := \left\{ i \middle| S_i > \frac{2}{\sqrt{3}} \right\}$. Then we have
  \begin{align*}
  &\mathbb{E}\sq*{\min_{0\leq k \leq K-1} \sq*{ \sum_{i\in B_k} |g_{k,i}| + \sum_{i\not\in B_k} \frac{g_{k,i}^2}{\sigma_i}} } \\
  & \qquad \qquad \qquad \leq \sqrt{\frac{3\norm{\vec L}_1}{N}}\sq*{f_0 - f_* + \frac{1}{2}}
  \end{align*}
\end{restatable}
\end{tcolorbox}
